Can 3D Pose be Learned from 2D Projections Alone?

3D pose estimation from a single image is a challenging task in computer vision. We present a weakly supervised approach to estimate 3D pose points, given only 2D pose landmarks. Our method does not require correspondences between 2D and 3D points to build explicit 3D priors. We utilize an adversarial framework to impose a prior on the 3D structure, learned solely from their random 2D projections. Given a set of 2D pose landmarks, the generator network hypothesizes their depths to obtain a 3D skeleton. We propose a novel Random Projection layer, which randomly projects the generated 3D skeleton and sends the resulting 2D pose to the discriminator. The discriminator improves by discriminating between the generated poses and pose samples from a real distribution of 2D poses. Training does not require correspondence between the 2D inputs to either the generator or the discriminator. We apply our approach to the task of 3D human pose estimation. Results on Human3.6M dataset demonstrates that our approach outperforms many previous supervised and weakly supervised approaches.

==> algorithm.tex <==


\begin{algorithm}
\KwIn{$\mathcal{X}$: the set of real 2D poses \newline
	%   $i = 1,...,\dfrac{\mathcal{X}}{M}$ \newline
	%$R_i$ is a random rotation matrix parameterized by the azimuth $\gamma \sim \mathcal{U}(0^\circ,360^\circ)$ and elevation $\phi \sim \mathcal{U}(0^\circ,20^\circ)$ \newline
	%$T = [0,0,d]$, where $d$ is a contant offset in the $z$-axis
    }
\KwOut{Final parameters $\theta_G$ and $\theta_D$}

\begin{algorithmic}

      \FOR {each iteration}
        \STATE Sample generator input batch $\bold{x}^G$ from $\mathcal{X}$
        \STATE Sample discriminator input batch $\bold{x}^D$ from $\mathcal{X}$
        \FOR {generator input skeleton $\bold{x}_i^G$}
          \FOR {each joint}
          	\STATE Estimate depths $z_i$ (Equations 1-2)
          	\STATE Back-project to 3D point $\bold{X}_i \leftarrow [z_i x_i,z_i y_i, z_i]$
          \ENDFOR
          \STATE Sample a random rotation $\bold{R}$
          \STATE Randomly rotate 3D skeleton $\bold{X}_i$ using $R$
          \STATE Project rotated 3D skeleton $P_i$ onto synthetic 2D landmarks $p_i$

        \ENDFOR
        \STATE Minimizing loss $V(D,G)$ w.r.t. $\theta_G$ over $\{p_i\}$
       	
        %\STATE Compute $s_i^D = D(\bold{x}_i^D; \theta_D)$ and $s_i^G = D(\bold{x}_i^G; \theta_D)$
        %\STATE Update $\theta_D$ using ADAM optimizer and discriminator component of the loss in equation (4)

        \STATE Maximizing the loss $V(D,G)$ w.r.t. $\theta_D$ over $\{p_i\}$
     and $\bold{x}^D$
     \ENDFOR
\end{algorithmic}
\end{algorithm}

